Towards Adversarial-Resilient Deep Neural Networks for False Data Injection Attack Detection in Power Grids

False data injection attacks (FDIAs) pose a significant security threat to power system state estimation. To detect such attacks, recent studies have proposed machine learning (ML) techniques, particularly deep neural networks (DNNs). However, most of these methods fail to account for the risk posed by adversarial measurements, which can compromise the reliability of DNNs in various ML applications. In this paper, we present a DNN-based FDIA detection approach that is resilient to adversarial attacks. We first analyze several adversarial defense mechanisms used in computer vision and show their inherent limitations in FDIA detection. We then propose an adversarial-resilient DNN detection framework for FDIA that incorporates random input padding in both the training and inference phases. Our simulations, based on an IEEE standard power system, demonstrate that this framework significantly reduces the effectiveness of adversarial attacks while having a negligible impact on the DNNs' detection performance.

==> background.tex <==
\section{Technical Background}
\label{sec:background}

\subsection{Power System State Estimation}


Enabled by the supervisory control and data acquisition (SCADA) techniques, power systems utilize state estimation to estimate the state of each bus, such as voltage angles and magnitudes, through analyzing the other measurements, such as the power of transmission lines, from the remote meters. We denote the vector of state variables as $\textbf{x} = \left [x_{1}, x_{2}, ..., x_{n} \right ]^{T}$, and the meters' measurements vector as $\textbf{z} = \left [z_{1}, z_{2}, ..., z_{m} \right ]^{T}$. The general state estimation process can be represented as follow:


\begin{equation}
\textbf{z} = \textbf{h}(\textbf{x}) + \textbf{e}
\end{equation}

where \textbf{e} is the measurement error vectors and \textbf{h} is a function of \textbf{x}. In practice, a DC power flow state estimation is usually used to decrease the process time cost. A DC model can be represented as equation (\ref{eq:dcModel}).

\begin{equation}
\textbf{z} = \textbf{H}\textbf{x} + \textbf{e}
\label{eq:dcModel}
\end{equation}

The matrix \textbf{$\textbf{H}_{m \times n}$} is determined by the configurations, topology and physical parameters of the power system.

In general, a weighted least squares estimation (WLS) approach is used to solve equation (\ref{eq:dcModel}). The estimated state vector $\hat{\textbf{x}}$ can then be computed through equation (\ref{eq:WLS}):

\begin{equation}
\textbf{$\hat{\textbf{x}}$} = (\textbf{H}^{T} \textbf{W} \textbf{H})^{-1} \textbf{H}^{T} \textbf{W} \textbf{z}
\label{eq:WLS}
\end{equation}

where matrix \textbf{$\textbf{W}$} is the covariance matrix of the meters' statistical measurement errors.


In practice, $\textbf{z}$ may contain bad measurements due to meter errors or cyber attacks. Therefore, state estimation integrates with a linear residual-based detection approach to remove faulty measurements according to the difference between $\textbf{z}$ and $\textbf{H} \textbf{$\hat{\textbf{x}}$}$. If the $L_{2}$-Norm of $\left \| \textbf{z} - \textbf{H} \textbf{$\hat{\textbf{x}}$} \right \|$ is larger than a threshold $\tau$ that is selected according to a false alarm rate, the measurement $\textbf{z}$ will be considered as polluted and be removed.


\subsection{False Data Injection Attack}


The FDIA enables an attacker to generate a false measurement vector $\textbf{a} = \left [ a_{1}, a_{2}, ..., a_{m} \right ]^{T}$ to be added to legitimate $\textbf{z}$, so that the polluted measurements will be $\textbf{z}_{a} = \textbf{z} + \textbf{a}$. \cite{liu2009false} shows that if the attacker knows $\textbf{H}$, she/he can construct $\textbf{a} = \textbf{H} \textbf{c}$ ($\textbf{c}$ represents the estimation error) that can bypass the fault detection in state estimation, as shown by equation (\ref{eq:FDIAPri}), where $\textbf{$\hat{\textbf{x}}$}_{bad}$ and $\textbf{$\hat{\textbf{x}}$}$ denote the estimated $\textbf{x}$ using $\textbf{z}_{a}$ and $\textbf{z}$ respectively.

\begin{subequations}
\begin{align}
\left \| \textbf{z}_{a} - \textbf{H} \textbf{$\hat{\textbf{x}}$}_{bad} \right \| \;\; &= \;\; \left \| \textbf{z} + \textbf{a} - \textbf{H}(\textbf{$\hat{\textbf{x}}$} + \textbf{c}) \right \| \\
 \;\; &= \;\; \left \| \textbf{z} - \textbf{H}\textbf{$\hat{\textbf{x}}$} + (\textbf{a} - \textbf{H}\textbf{c}) \right \| \\
 \;\; &= \;\; \left \| \textbf{z} - \textbf{H}\textbf{$\hat{\textbf{x}}$} \right \| \leq \tau
\end{align}
\label{eq:FDIAPri}
\end{subequations}

Meanwhile, equation (\ref{eq:FDIAgen}) from \cite{liu2009false} provides an efficient way to generate a valid vector $\textbf{a}$, where $\textbf{P} = \textbf{H}(\textbf{H}^{T}\textbf{H})^{-1}\textbf{H}^{T}$ and matrix $\textbf{B} = \textbf{P} - \textbf{I}$.

\begin{subequations}
\begin{align}
\textbf{a} = \textbf{H}\textbf{c} \;\; &\Leftrightarrow\;\; \textbf{P}\textbf{a} = \textbf{P}\textbf{H}\textbf{c} \Leftrightarrow \textbf{P}\textbf{a} = \textbf{H}\textbf{c} \Leftrightarrow \textbf{P}\textbf{a} = \textbf{a} \\
\;\; &\Leftrightarrow\;\; \textbf{P}\textbf{a} - \textbf{a} = \textbf{0} \Leftrightarrow  (\textbf{P}-\textbf{I})\textbf{a} = \textbf{0} \\
\;\; &\Leftrightarrow\;\; \textbf{B}\textbf{a} = \textbf{0}
\end{align}
\label{eq:FDIAgen}
\end{subequations}

Equation (\ref{eq:FDIAgen}c) indicates that $\textbf{a}$ is a solution of the homogeneous equation $\textbf{B}\textbf{X} = \textbf{0}$. If an attacker compromised $k$ measurements in $\textbf{z}$, and there will be $k$ non-zero elements in $\textbf{a}$. Equation (\ref{eq:FDIAgen}c) will then become:

\begin{equation}
\textbf{B'}\textbf{a'} = \textbf{0}
\label{eq:FDIAgenSim}
\end{equation}

where $\textbf{B'}_{m \times k}$ and $\textbf{a'}_{m \times k}$ are corresponding columns and rows sampled from $\textbf{B}$ and $\textbf{a}$ respectively according to the $k$ compromised measurements. \cite{liu2009false} proves that as long as $k > m-n$, non-zero $\textbf{a}$ always exists.


